Feynman-Kac Derivatives Pricing on the Full Forward Curve

This paper introduces a no-arbitrage, Monte Carlo-free approach to pricing path-dependent interest rate derivatives. The Heath-Jarrow-Morton model gives arbitrage-free contingent claims prices but is infinite-dimensional, making traditional numerical methods computationally prohibitive. To make the problem computationally tractable, I cast the stochastic pricing problem as a deterministic partial differential equation (PDE). Finance-Informed Neural Networks (FINNs) solve this PDE directly by minimizing violations of the differential equation and boundary condition, with automatic differentiation efficiently computing the exact derivatives needed to evaluate PDE terms. FINNs achieve pricing accuracy within 0.04 to 0.07 cents per dollar of contract value compared to Monte Carlo benchmarks. Once trained, FINNs price caplets in a few microseconds regardless of dimension, delivering speedups ranging from 300,000 to 4.5 million times faster than Monte Carlo simulation as the state space discretization of the forward curve grows from 10 to 150 nodes. The major Greeks-theta and curve deltas-come for free, computed automatically during PDE evaluation at zero marginal cost, whereas Monte Carlo requires complete re-simulation for each sensitivity. The framework generalizes naturally beyond caplets to other path-dependent derivatives-caps, swaptions, callable bonds-requiring only boundary condition modifications while retaining the same core PDE structure.

==> results/latex_diss/error_metrics_k100.tex <==
\begin{table}[htbp]
\centering
\caption{Error Metrics for FINN vs Monte Carlo at $K=100$}
\label{tab:error_metrics_k100}
\begin{tabular}{lc}
\hline
\textbf{Metric} & \textbf{Value} \\
\hline
Mean Absolute Error (MAE) & $0.000375$ \\
Root Mean Squared Error (RMSE) & $0.000548$ \\
Maximum Error & $0.003229$ \\
Mean Signed Error (Bias) & $0.000091$ \\
$R^2$ Coefficient & $0.993630$ \\
\hline
\multicolumn{2}{l}{\textit{Computational Performance}} \\
\hline
MC Time per Contract (s) & $5.435753$ \\
FINN Time per Contract (s) & $0.000002$ \\
Speedup Factor & $2522035.4\times$ \\
\hline
\multicolumn{2}{l}{\textit{Monte Carlo Parameters}} \\
\hline
MC Paths & $10,000$ \\
MC Time Steps & $1,000$ \\
Average MC Std Error & $0.000055$ \\
\hline
\multicolumn{2}{l}{\textit{Test Set}} \\
\hline
Number of Contracts & $1,000$ \\
Discretization ($K$) & $100$ \\
\hline
\end{tabular}
\end{table}


==> results/plots_diss/error_metrics_k100.tex <==
\begin{table}[htbp]
\centering
\caption{Error Metrics for FINN vs Monte Carlo at $K=100$}
\label{tab:error_metrics_k100}
\begin{tabular}{lc}
\hline
\textbf{Metric} & \textbf{Value} \\
\hline
Mean Absolute Error (MAE) & $0.000375$ \\
Root Mean Squared Error (RMSE) & $0.000548$ \\
Maximum Error & $0.003229$ \\
Mean Signed Error (Bias) & $0.000091$ \\
$R^2$ Coefficient & $0.993630$ \\
\hline
\multicolumn{2}{l}{\textit{Computational Performance}} \\
\hline
MC Time per Contract (s) & $5.435753$ \\
FINN Time per Contract (s) & $0.000002$ \\
Speedup Factor & $2522035.4\times$ \\
\hline
\multicolumn{2}{l}{\textit{Monte Carlo Parameters}} \\
\hline
MC Paths & $10,000$ \\
MC Time Steps & $1,000$ \\
Average MC Std Error & $0.000055$ \\
\hline
\multicolumn{2}{l}{\textit{Test Set}} \\
\hline
Number of Contracts & $1,000$ \\
Discretization ($K$) & $100$ \\
\hline
\end{tabular}
\end{table}


==> results/plots_diss/timing_table.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|ccc|c|}
\hline
$K$ & MC Time & FINN Time & Speedup Multiple & MAE \\
\hline
$10$ & $0.96$ & $3.10 \times 10^{-6}$ & $311{,}366$ & $8.73 \times 10^{-4}$ \\
$25$ & $1.18$ & $4.25 \times 10^{-6}$ & $276{,}943$ & $6.25 \times 10^{-4}$ \\
$35$ & $1.40$ & $5.45 \times 10^{-6}$ & $257{,}440$ & $5.69 \times 10^{-4}$ \\
$50$ & $1.92$ & $5.91 \times 10^{-6}$ & $324{,}690$ & $5.17 \times 10^{-4}$ \\
$75$ & $3.49$ & $2.45 \times 10^{-6}$ & $1{,}421{,}537$ & $9.42 \times 10^{-4}$ \\
$100$ & $5.44$ & $2.16 \times 10^{-6}$ & $2{,}522{,}035$ & $3.75 \times 10^{-4}$ \\
$125$ & $8.22$ & $2.53 \times 10^{-6}$ & $3{,}245{,}742$ & $7.98 \times 10^{-4}$ \\
$150$ & $10.08$ & $2.23 \times 10^{-6}$ & $4{,}522{,}638$ & $4.03 \times 10^{-4}$ \\
\hline
\end{tabular}
\caption{{Computational performance and accuracy across discretization phases. MC Time and FINN Time are in seconds per contract. Speedup Multiple is the ratio of MC Time to FINN Time. MAE (Mean Absolute Error) measures the difference between FINN and Monte Carlo prices.}}
\label{tab:timing}
\end{table}

